Compositional Visual Generation and Inference with Energy Based Models

A vital aspect of human intelligence is the ability to compose increasingly complex concepts out of simpler ideas, enabling both rapid learning and adaptation of knowledge. In this paper we show that energy-based models can exhibit this ability by directly combining probability distributions. Samples from the combined distribution correspond to compositions of concepts. For example, given a distribution for smiling faces, and another for male faces, we can combine them to generate smiling male faces. This allows us to generate natural images that simultaneously satisfy conjunctions, disjunctions, and negations of concepts. We evaluate compositional generation abilities of our model on the CelebA dataset of natural faces and synthetic 3D scene images. We also demonstrate other unique advantages of our model, such as the ability to continually learn and incorporate new concepts, or infer compositions of concept properties underlying an image.

==> figText/andor.tex <==
% \begin{figure}[h]
% \centering
% \begin{minipage}{0.45\textwidth}
%     \includegraphics[width=1.0\textwidth]{fig/celeba_or.pdf}
%     \caption{Examples of concept addition on joint attributes (represented by addition of energy) of not smiling/female and smiling/male. EBMs are able to reliably support concept addition (generation of either one concept or the other) even when the concept itself is compound.}
%     \label{fig:celeba_or}
% \end{minipage}\hfill
% \begin{minipage}{0.45\textwidth}
%     \includegraphics[width=1.0\textwidth]{fig/celeba_neg.pdf}
%     \caption{Examples of concept negation on the attributes of smiling / female. When negating the female energy in combination with the smiling energy function, we are able to generate photos of males that are smiling}
%     \label{fig:celeba_not}
% \end{minipage}\hfill
% \end{figure}


% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=0.9\textwidth]{fig/andor.pdf}
% \end{center}
% \vspace{-10pt}
% \caption{\small (a) Examples of concept disjunction on joint attributes (represented by conjunction of energy) of not smiling+female and smiling+male. EBMs are able to reliably support concept disjunction (generation of either one concept or the other) even when the concept itself is compound. 
% (b) Examples of concept negation on the attributes of smiling female. When negating the female energy in combination with the smiling energy function, we are able to generate photos of males that are smiling.}
% \label{fig:andor}
% \end{figure*}



\begin{wrapfigure}{L}{0.45\textwidth}
\begin{center}
\includegraphics[width=0.45\textwidth]{fig/icml/result.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Examples of recursive compositions of disjunction, conjunction, and negation on the CelebA dataset. 
% \im{say these can be nested.} 
}
\label{fig:andor}
\vspace{-10pt}
\end{wrapfigure}

==> figText/celeba_combine.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\textwidth]{fig/celeba_combine.pdf}
\end{center}
\caption{Examples of combination of different attributes on CelebA via summation of energies. Each row adds an additional energy function attribute. For example, images on the first row are only conditioned on young while images on the last row are conditioned on young, female, smiling and wavy hair.}
\label{fig:celeba_combine}
\end{figure}

==> figText/continual.tex <==
% \begin{figure}[!b]
% \begin{center}
% \includegraphics[width=1\textwidth]{fig/continual.pdf}
% \end{center}
% \caption{Examples of continual learning of concepts. The first energy function learns to generate different position squares. A second energy function then learns to construct different shapes at a target position. Finally, a third energy function is able to be learned to modulate modulate the shape / position of generations.}
% \label{fig:continual}
% \end{figure}


\begin{figure}[!b]
\begin{center}
\includegraphics[width=1\textwidth]{fig/continual2.pdf}
\end{center}
\caption{Examples of continual learning of concepts. The first row shows generation of the first energy function trained on different position squares conditioned on different positions. The second row shows a second energy function then learns to construct different shapes at a target position, with the first energy function, when conditioned on the sphere shape. Finally, the third row shows a third newly learned energy function is able to be learned to modulate the previously learned energy functions with different colors.}
\label{fig:continual}
\end{figure}

==> figText/mujoco_combine.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1\textwidth]{fig/mujoco_combine.pdf}
\end{center}
\caption{Examples of combination of different attributes on Mujoco via summation of energies. Each column adds an additional energy function attribute. For example, images on the first column are only conditioned on shape while images on the last column are conditioned on shape, position, size and color.}
\label{fig:mujoco_combine}
\end{figure}

==> figText/multi_view.tex <==
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.5\textwidth]{fig/multiview.pdf}
% \end{center}
% \caption{The influence of multiple observations, images generated under different lighting conditions and camera heights, on EBMs. The position prediction errors decrease when the number of input images increases on different steps.}
% \label{fig:multiview}
% \end{figure}



\begin{figure}[t]
\begin{center}
\includegraphics[width=0.42\textwidth]{fig/icml/multiobj.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Concept inference from multiple observations. Multiple images are generated under different size, shape, camera view points, and lighting conditions.
The position prediction error decreases when the number of input images increases with different Langevin Dynamics sampling steps.}
\label{fig:multiview}
\vspace{-5pt}
\end{figure}


% \begin{wrapfigure}{l}{0.5\textwidth}
%     \includegraphics[width=\linewidth]{fig/multiview2.pdf}
%   \caption{The influence of multiple observations on EBMs. The multiple images are generated under different lighting conditions and camera heights. The position prediction errors decrease when the number of input images increases on different steps.}
% \end{wrapfigure}


==> figText/step.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.44\textwidth]{fig/icml/step.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Examples of generated images with varying number of Langevin Dynamics sampling steps. Larger number of steps leads to more realistic images.}
\label{fig:step}
\vspace{-10pt}
\end{figure}

==> figText/twocubes.tex <==
% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=1\textwidth]{fig/twocubes3.pdf}
% \end{center}
% \caption{Energy based model trained on single cubes and test on two cubes. The RGB images and Grey images are the input images and output energy maps respectively. The EBM works well on unseen two cubes images.}
% \end{figure}


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=1\textwidth]{fig/twocubes4.pdf}
% \end{center}
% \caption{Energy based model trained on single cubes and test on two cubes. The RGB images and Grey images are the input images and output energy maps respectively. The EBM works well on unseen two cubes images.}
% \end{figure}


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=1\textwidth]{fig/twocubes6.pdf}
% \end{center}
% \caption{Energy based model trained on single cubes and test on two cubes. The RGB images and Grey images are the input images and output energy maps respectively. The EBM works well on unseen two cubes images.}
% \end{figure}



\begin{figure}
\begin{center}
\includegraphics[width=0.4\linewidth]{fig/twocubes6.pdf}
\end{center}
\vspace{-5pt}
\caption{\small Concept inference of multiple objects with EBM trained on single cubes and tested on two cubes. The color image is the input and in grayscale is the output energy map over all positions. The energy map of two cubes correctly shows the bimodality which is close to the summation of the front two energy maps.}
 \label{fig:twocubes}
 \vspace{-10pt}
\end{figure}



==> text/evaluation__Yilun_Du_s_conflicted_copy_2020-06-11_.tex <==

\section{Experiments}
We perform empirical studies to answer the following questions: Can EBMs exhibit concept compositionality, such as concept negation, conjunction, and disjunction, in generating images? Can we take advantage of concept combinations to learn new concepts in a continual manner? Does explicit factor decomposition enable better generalization? Can we perform inference across multiple inputs?

\subsection{Setup}
We perform experiments on 64x64 different object scenes rendered in Mujoco \citep{Todorov2012MuJoCo} and the 128x128 CelebA dataset. For scenes rendered in Mujoco, we generate a central object of shape either sphere, cylinder, or box of varying size and height, with some number of (specified) additional background objects. Images are generated with varying lighting and objects.

We use the ImageNet32x32 architecture and ImageNet128x128 architecture from \citep{du2019implicit} with the Swish activation \citep{ramachandran2017searching} on Mujoco and CelebA datasets. Models are trained on Mujoco datasets for up to 1 day on 1 GPU and for 1 day on 8 GPUs for CelebA. More training details and model architecture can be found in and \ref{appendix:model} and \ref{appendix:training_detail}.


\input{figText/andor.tex}
\subsection{Compositional Generation}
We evaluate EBMs on generation images via compositionality operations of the previous section. 
% \jm{When you says "to what extend", is there any quantitative results available?}
% \im{Venn diagrams of combination / addition / negation alongside small image samples from each region could be really helpful}

\myparagraph{Concept Conjunction} We find that in \fig{fig:celeba_mujoco_combine} (a) that EBMs are able to combine independent concepts of age, gender, smile, and wavy hair with each additional attribute allowing more precise generation. Similarily, we find in \fig{fig:celeba_mujoco_combine} (b) that EBMs are able to combine independent concepts of shape, position, size, and color together to generate more precise generations.

\myparagraph{Concept Disjunction} We also find that EBMs are able to combine concepts additively (generate images that are concept A or concept B) as shown in \fig{fig:andor} (a). By constructing sampling using logsumexp, EBMs are able to either sample an image that is not smiling female or smiling male, where both not smiling female and smiling male are specified through the conjunction of energies of the two different concepts. This result also shows that concept disjunction can be chained on top of other operators such as concept conjunction.

\myparagraph{Concept Negation} We further generate concepts that are the opposite of the trained concept in \fig{fig:andor} (b), where we find that negating female, in combination with smiling leads to generation of a smiling male. Furthermore, we note that the ability of concept conjunction, disjunction, and negation allows us to flexibly specify any set of pairwise concepts.

\myparagraph{Multiple Object Combination} 
Finally, we explore the use of an EBM to model single object-based concepts. To investigate this, we constructed a dataset consisting of a central green cube with size and position annotations, in conjunction with large amount background clutter objects (which are not green), in which we trained a conditional EBM.

Despite the fact that the training dataset does not have any other green cubes, we find that adding two conditional EBMs conditioned on two different position and sizes, allowing us to selectively generate two different cubes in \fig{fig:continual_obj_com1}. Furthermore, we find that such generation is able to satisfy the constraints of the dataset. For example, when two conditional cubes are too close, the conditionals EBMs are able to default to generating one cube.


\input{figText/continual_obj_comb.tex}
\input{figText/gen_size_pos.tex}
\input{figText/gen_precent.tex}

\subsection{Continual Learning}

An important ability humans are endowed with is the ability to both continually learn new concepts, and to extrapolate existing concepts in combination with previously learned concepts. We evaluate to what extent compositionality in EBMs enables this through the following continual learning process:
\begin{enumerate}
    \myitem We first train an EBM for position based generation by training it on a dataset of cubes at various positions of a fixed color.
    \myitem Next we train an EBM for shape based generation, by training the model in combination with the positional model to generate images on a dataset of different shapes (through summation) at different positions, but with the position based EBM fixed.
    \myitem Finally we train an EBM for color based generation, by training the model in combination with both positional and shape models to generate images on a dataset of different shapes at different positions and colors (through summation).  Again we fix both position and shape EBMs, and only train the color based generation.
\end{enumerate}
We show in \fig{fig:continual_obj_com2} that this allow us to \textbf{extrapolate} our learned models for position and shape to generate different position shapes of various colors. The first column of \fig{fig:continual_obj_com2} shows the generations of a positional model, while the second column shows the generation of both positional and shape models, and the third column columns shows the generation of position, shape, and color models. Even though the positional model has only seen cubes of a particular color at a particular position, and color model shapes of a particular color, the third column illustrates that the composition of all three models is able to allow the generation of different colored shapes at various positions.



%\jm{Section 3.4 and 3.5 are a bit confusing. The should be organized in a better way: they both talk about ``out-of-training-distribution'' generalization. I suggest dividing them clearly into two parts: concept classification and image generation (there is one paragraph in sec 3.5 which is actually talking about image generation I believe...).}


\subsection{Cross Product Generalization}
% \jm{A venn diagram-like thing may help exlaining the settings here}

Humans are endowed with the ability to extrapolate novel concept combinations when only a limited number of combinations were originally observed. For example, despite never having seen a purple person, one might compose what such a person looks like.

We evaluate the extent to which EBMs, which allow us to factorize generation into different concepts, can help us extrapolate. To test this, we construct a dataset of mujoco scene images with spheres of all possible sizes appearing in an increasing percentage of positions starting from top right corner and spheres of only large size appearing in all remaining positions (see left Figure \ref{fig:gen_precent} for illustration), \eg $1\%$ means only $1\%$ of positions starting from top right corner with all sphere sizes are used for training. At test time, we evaluate generation of spheres of all sizes at positions not seen at training time. Such a task requires the model to extrapolate the learned position and size concepts in novel combinations.

We train two EBMs on this dataset - one conditioned on position latent and trained only on large sizes and another conditioned on size latent and trained at the aforementioned percentage of positions. Conjunction of the two EBMs is fine-tuned on this dataset using gradient descent on Equation \ref{eq:mce}. We compare this composed model with a baseline holistic model conditioned on both position and size jointly, trained on the same position/size combinations, and optimized directly for Mean Squared Error loss. Both models use the same architecture and number of parameters (described in Appendix).

Qualitatively, \fig{fig:gen_precent} illustrates that by learning an independent model for each concept factor, it is possible to combine them to form images from very few combination examples. For reference, both combined and baseline models generate accurate images when given examples of all combinations.

To evaluate generation performance quantitatively, we train a regression model that outputs both the position and size of a generated sphere image. We show errors in regressed size and position from combination and baseline models from ground truth in figure \fig{fig:gen_size_pos}. We find that EBMs are able to extrapolate both position and size better than a baseline joint model. We note that both models obtain less positional generation error at 1\% data as opposed to 5\% or 10\% of data. This result is due the make-up of the data -- with 1\% data, only 1\% of the rightmost sphere positions have different size annotations, so failed extrapolation causes models to generate large spheres at the conditioned position. Once there are more different size sphere annotations from data, models either collapse to an existing size or position, leading to a higher error.


\input{figText/diff_cond.tex}
\input{figText/multi_view.tex}

\subsection{Compositional Concept Inference}
%\jm{Is it true you want to talk about compositional concept classification? The ``compositional inference'' is a bit confusing and I can't distinguish this section (by title) with sec 3.2. Also, I suggest using multiple paragraph titles to make different experiments separate more clearly.}
In addition to generation, EBMs can be used to infer the underlying concept latent factors that gave rise to a particular image. We show this process can also infer compositions of underlying factors.

\myparagraph{Concept Parameter Inference}
To infer underlying concept parameters given an image, we minimize concept energy with respect to these parameters (Equation \ref{eq:min_infer}). To evaluate inference accuracy, we generate a mujoco scene image dataset with speheres and cubes at all possible positions under varying lighting and objects. We train an EBM on this dataset using our standard objective and evaluate Mean Absolute Error between inferred object position and ground truth position.

We construct a variety of test datasets that specifically use combinations of concept not seen during training to test generalization of position inference. \emph{``Color''} refers to a test dataset with object colors never before seen in training. \emph{``Light''} is a test dataset with different light sources. \emph{``Size''} is a test dataset with object sizes not seen during training and \emph{``Type''} dataset consists of cylinder images while the training images are only spheres or cubes.
%We approximate Maximum A Posteriori Estimation inference of positions by exhaustive sampling over a grid of possible values. 

% \begin{equation}
%     \text{error} = (\left| \hat{x_1} - x_1 \right| + \left| \hat{y_1} - y_1 \right|) / 2.
% \end{equation}

We compare EBMs with a baseline ResNet model \citep{he2016deep} (with the same architecture as the EBM) trained directly to regress on true position and a conditional generative baseline PixelCNN \citep{oord2016pixel}. \tbl{tbl:compositional_inference} shows the comparisons of EBMs with different number of Langevin Dynamics sampling steps and the ResNet model.
% The number of Langevin sampling steps used during training significantly improves inference.
EBMs with larger Langevin sampling steps outperform the ResNet model, generalizing significantly better. Furthermore, larger numbers of sampling steps leads to better generation quality as shown in \fig{fig:multiview} (b). This suggests that many figures in this paper (which are trained with 40 sampling steps) can likewise see a large boost in the generation quality. 

% Furthermore, we find that the resulting regression is highly \textbf{robust} and significantly outperforms the ResNet architectures in \tbl{tbl:compositional_inference}  to test datasets with changes of color, lighting, size, and type. ``Color'' refers to a test dataset where component shapes have a novel color. ``Light'' refers to a test dataset where the light source changes and ``Size'' refers to a test dataset where based shape size changes. Finally ``Type'' refers to a test dataset where the evaluated shapes are cylinders.  % We provide examples of our original and modified test datasets in the appendix.


\input{figText/twocubes.tex}
% diff = np.mean(np.abs(label_pred - pos_label.squeeze())).
\myparagraph{Inference from Multiple Observations}
Another advantage of compositionality in EBMs is the ability to effectively make use of multiple observations when making inferences. We evaluate this ability by measuring the Mean Absolute Error in position when given successively more images with varying of objects and lighting angles. We display results in Figure \ref{fig:multiview} (a) and find that our model is able to integrate multiple observations to improve prediction performance.

% One advantage of our EBMs is it can average over multiple energy maps and generate reasonable energy maps to show the position of objects. 

% On each position, we generate several images with different light conditions and camera heights. 
% The test errors using one, two, and three images are 4.276, 3.793, and 3.721 respectively.
\myparagraph{Inference of Multiple Objects}
We also investigate the role of compositionality in generalizing inference to multiple objects. Given EBMs trained on images of a single object, we test on images with multiple objects (not seen in training). We plot energies over possible position values in Figure \ref{fig:twocubes} as well as energy maps over each individual cube. We find that EBMs naturally form bimodal object position distributions that match the summation of distributions for each individual object. We need to specify the number of scene objects for this inference process.


